KHOVID: Interoperable Privacy Preserving Digital Contact Tracing

During a pandemic, contact tracing is an essential tool to drive down the infection rate within a population. To accelerate the laborious manual contact tracing process, digital contact tracing (DCT) tools can track contact events transparently and privately by using the sensing and signaling capabilities of the ubiquitous cell phone. However, an effective DCT must not only preserve user privacy but also augment the existing manual contact tracing process. Indeed, not every member of a population may own a cell phone or have a DCT app installed and enabled. We present KHOVID to fulfill the combined goal of manual contact-tracing interoperability and DCT user privacy. At KHOVID's core is a privacy-friendly mechanism to encode user trajectories using geolocation data. Manual contact tracing data can be integrated through the same geolocation format. The accuracy of the geolocation data from DCT is improved using Bluetooth proximity detection, and we propose a novel method to encode Bluetooth ephemeral IDs. This contribution describes the detailed design of KHOVID; presents a prototype implementation including an app and server software; and presents a validation based on simulation and field experiments. We also compare the strengths of KHOVID with other, earlier proposals of DCT.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> system_overview.tex <==
\revision{\subsection{\sysName Architecture}}
% \subsection{COVID Detector Architecture}
% As shown in Figure 1, \sysName is formed by three components: RedZone Collector, Risk Checker, and Risk Interpreter. Risk Checker is a smartphone app that locally logs a user’s trajectory   and its encounter with other \sysName phones in the past two weeks, where the two-week time span is the maximum incubation period. If a user of Risk Checker is tested positive with COVID-19 infection, he can voluntarily let the app upload his past trajectories and encounter information to the RedZone Collector through a strict privacy protection mechanism. Manual contact tracing  data about patients’ whereabouts can also be uploaded to RedZone Collector by healthcare authorities using a similar privacy-preserving mechanism.  The RedZone Collector integrates all these patient input data in a privacy-friendly manner. A person, who wants to evaluate her own risk level of contracting the disease from confirmed cases, can query the RedZone Collector to compare her own phone’s trajectory and encounter records with the integrated patient trajectory and encounter data from the RedZone Collector. The intersections of a user’s past with aggregated patient history can then be mapped towards a risk level value. The risk level is defined as a weighted summation of the number of intersections, where a highest weight will be given if the user was present with known patients at a location at the same time, and a lower weight is used if the user was further separated from active patients in distance and/or in time. The risk level can be interpreted by the Risk Interpreter to provide a risk analysis. The entire above COVID-Detector operations are carried out under strong privacy protection schemes, so that both patient and general public’s trajectories are never exposed or shared to any party (See Section \ref{section:system} for details).

As shown in Figure~\ref{fig:overview}, \sysName design involves four parties: (1) patients, (2) normal users, (3) \redzone, and (4) \riskInter. \riskInter is a central server that is responsible for key distributing and ciphertext decryption. \riskInter generates a group of Paillier public/private key pair $(pk,sk)$.  The public key $pk$ is distributed to all users and RedZone Collector. Private key $sk$ is kept as a secret only known to \riskInter, which means \riskInter is the only party who can decrypt a Paillier ciphertext in the system. \redzone is another central server that stores data and conducts contact tracing history comparisons between normal users with patients. Both patients and normal users have downloaded the \sysName smartphone app that locally logs a user’s trajectory and its encounter with other \sysName phones in the past two weeks, where the two-week time span is the maximum incubation period. 

Once a normal user is tested positive with COVID-19 and becomes a patient, he/she can voluntarily let the app upload his past trajectories and encounter information to \redzone. The uploaded information are under strict privacy protection as the information are masked using k-anonymity and  Paillier encryption algorithm before uploading. Manual contact tracing data about patients’ whereabouts can also be uploaded to \redzone by healthcare authorities using the same privacy-preserving mechanism. A normal user, who wants to evaluate his own exposure risk of contracting the disease from confirmed cases, can query \redzone to privately compare his own phone’s trajectory and encounter records with the masked patient trajectory and encounter data from \redzone. The private comparison results are in homomorphically encrypted form and their values are never revealed to 
\redzone.  The normal user who initiates the private comparison obtained the comparison results in encrypted form and sent the results to \riskInter, which decrypts the comparison results, converts it to an exposure risk metric to further improve privacy protection to patients, and returns the metric to the normal user. The entire above COVID-Detector operations are carried out under strong privacy protection schemes, so that both  patients' and normal users' trajectories are not exposed or shared with each other, the servers or any other parties. (See Section \ref{section:geo-method} and \ref{sec:BLE-method} for details).



% From prof.Yang:  Too specific to geo side, does not fit the bluetooth side

%The intersections of a user’s past with patient history can then be mapped towards an exposure risk value. The exposure risk is defined as a weighted summation of the number of intersections, where the highest weight will be given if the user was present with known patients at a location at the same time, and a lower weight is used if the user was further separated from active patients in distance and/or in time. The calculation of exposure risk is formed into a set of homomorphic operations, thus when an exposure risk is returned to the normal user, it is in the ciphertext and \redzone is not aware of what the exposure risk is. The exposure risk then can be passed from the normal user to \riskInter for further risk analysis. 

\begin{figure*}[ht]
    \centering
    \includegraphics[scale=0.5]{fig/COVID Detector overview.pdf}
    \caption{An overview of \sysName System }
    \label{fig:overview}
\end{figure*}

%\subsection{Problem Definition}
%\subsection{Notations}
% To ensure ease of discussion, the following terms are defined for the rest of the paper: 
% \begin{enumerate}
%     \item \textit{Patients}: Persons who have been medically diagnosed with COVID-19 and use our contact tracing app. Patients decide to report their past trajectories as well as encounter information to the RedZone Collector after they got diagnosed. 
%     \item \textit{Contact}: A person that has been in close proximity with a patient sometime during the past 14 days of incubation period. \cite{cryptoeprint:2020:672}. 
%     \item \textit{Exposure risk}: Exposure risk level reflects the probability that a person has been exposed to the virus. The more past contacts that a person has with patients, the higher the risk level is. 
    
%     \item \textit{Normal user}: A user of our contact tracing app, who is not diagnosed with COVID-19. A normal user may use our app to  check his/her exposure risk level to the virus.
% \end{enumerate}

% \subsection{System Assumption}
% COVID Detector relies on two servers, RedZone Collector and Risk Interpreter.  We assume both servers satisfy honest-but-curious assumptions and are not colluding with each other.  Specifically, this means: 
% \begin{enumerate}
%     \item Both servers will follow the designed protocols.
%     \item Both  servers will not collude with each other. This means RedZone Collector won’t share any trajectory information to Risk Interpreter, and Risk Interpreter will neither deliver the private key nor provide risk level decryption to the RedZone Collector. 
%     \item Both servers may attempt to derive sensitive user privacy information from information they received. 
%     \item Both servers have no control over the app. This means the deciphered information will not sent to RedZone Collector, and the user trajectories will not sent to Risk Interpreter.
%     % \item Both servers will not collude with app users. This means except normal query requests, RedZone Collector will not ask app users to decrypt ciphertext for it, and Risk Interpreter will not ask app users to upload trajectory information to it. 

% \end{enumerate}


%\subsection{Threat Model and Privacy Goal}
%In this section, we introduce the threat model and define the privacy goals of the proposed system.


% \subsection{Threat Model}
% We consider three attackers in our threat model:
% \begin{itemize}
%     \item \textit{App user} refers to anyone with the COVID-Detector app installed in their smartphone. An app user based attacker is an active malicious user who is actively participating in the protocol by injecting real or malicious messages. For example, an malicious attacker can fake as a patient and send spurious patient location trajectories to RedZone Collector. 
    
%     \item \textit{Servers}, including  RedZone Collector and Risk Interpreter,  are maintained by the health authority or government, who is responsible for the operation and data on both the RedZone collector and Risk Interpreter. We consider an honest-but-curious server who is a legitimate participant that follows the protocol but may want to derive sensitive user information based on received protocol messages. For example, the RedZone collector may learn user's home address or build social graphs from the uploaded location information.  We assume that RedZone Collector and Risk Interpreter do not collude with each other.
    
%     \item \textit{Passive observers} may listen to all communication between app users and servers. For example, a passive observer may try to differentiate between positive and negative exposure risk level using traffic analysis.  
% \end{itemize}

% We assume that there is an authenticated and encrypted communication channel between each client and server, for example, using TLS~\cite{}. 

% When evaluating the threat from attackers, it is important to define the types of adversaries. Attackers can be divided into three categories: \textit{honest-but-curious attackers}, \textit{malicious attackers}, and \textit{passive observers}. 
% \begin{itemize}
%     \item \textit{Honest-but-curious servers} usually refer to central servers, they follow the protocols but also try to learn as much information as they can.  For example, the RedZone collector may try to learn patients’ home addresses and build social graphs from patients’ reported information. 
%     \item \textit{Malicious users} can use any possible strategies like replaying or modifying messages to deviate from protocols. Malicious attackers mainly come from App users. For an infected user who has a malicious attempt, he can modify the trajectory history reported to the RedZone collector, to make public panic. For an uninfected malicious user, he can either pretend to be an infected user and upload malicious messages to make public panic, or just be curious to figure out whether somebody he knows has been infected. 
%     \item \textit{Passive observers} can be governments or internet service providers, both of them have the capability to observe all the communications between parties participating in the protocol, and their goal is to learn as much information as they can. For example, they may differentiate positive/negative exposure risk levels by implementing traffic analysis.
% \end{itemize}
 
% Regarding the computation and storage resources, we assume both \textit{honest-but-curious attackers} and \textit{passive observers} can have unlimited resources since they can be nation-state attackers or tech giants. \texit{Malicious users} can be individuals or a malicious organization, in this paper \textit{malicious users} are also assumed to have unlimited computation and storage resources. 

% \subsection{Privacy Goal}
% Based on the threat model discussed above, an ideal contact tracing system should meet the following privacy goals. 
% \subsubsection{Privacy for Patients}
% Diagnosed patients voluntarily upload their trajectory information to the RedZone collector, any patients’ personal information (identity, past trajectories, home address, etc.) should not be revealed to other participants in the protocols, including RedZone collector, Risk interpreter and normal users. In addition, patients’ personal information should not be leaked to \textit{passive observers} either. 

% \subsubsection{Privacy for Normal Users}
% Normal users will compare their own trajectories with the data on the RedZone collector, and ask Risk interpreter to analyze their exposure risk level. During these operations, neither RedZone collector nor Risk Interpreter can infer normal users’ personal information as well as their real exposure risk level. The exposure risk level can only be known by the normal user. 

% \subsubsection{Correctness}
% The system should make sure reported information comes from real diagnosed patients, and their information is as accurate as possible, the reported messages should not be modified by malicious users. 
